When Celebrities Speak: A Nationwide Twitter Experiment Promoting Vaccination in Indonesia

Celebrity endorsements are often sought to influence public opinion. We ask whether celebrity endorsement per se has an effect beyond the fact that their statements are seen by many, and whether on net their statements actually lead people to change their beliefs. To do so, we conducted a nationwide Twitter experiment in Indonesia with 46 high-profile celebrities and organizations, with a total of 7.8 million followers, who agreed to let us randomly tweet or retweet content promoting immunization from their accounts. Our design exploits the structure of what information is passed on along a retweet chain on Twitter to parse reach versus endorsement effects. Endorsements matter: tweets that users can identify as being originated by a celebrity are far more likely to be liked or retweeted by users than similar tweets seen by the same users but without the celebrities' imprimatur. By contrast, explicitly citing sources in the tweets actually reduces diffusion. By randomizing which celebrities tweeted when, we find suggestive evidence that overall exposure to the campaign may influence beliefs about vaccination and knowledge of immunization-seeking behavior by one's network. Taken together, the findings suggest an important role for celebrity endorsement.

==> Endorsement.tex <==


\section{The Value of Endorsement}\label{sec:value_endorsement} 


This section explore our main results that characterize the value of endorsement per se. The key idea is that if a celebrity is known to be involved in passing a message, or have authored a message, this  provide scope for an endorsement effect. 
The very fact that the celebrity's identity is tied to the message may make others more likely to pass on the message, thereby accelerating diffusion. Similarly, a message explicitly listing a source may be more likely to be passed on if viewed as more credible, whereas if it lacks a source, this may impede diffusion. On the other hand, source inclusion may impede diffusion, say if passing such a benefit accrues the sender less social value.  Further, multiple exposures as compared to a single exposure may lead to more passing of information.

To untangle these mechanisms, in this section we use the variation we induced at the the tweet level---i.e., the randomly induced variation in who tweeted or retweeted what when. Since the variation we explore here is much finer, our outcome variables must also be at the level of the individual tweet.\footnote{In particular, the randomizations we exploit here are within-celebrity, and hence within-Phase. Therefore we cannot use other tweet-level randomizations in this section to look at  offline beliefs or behavior.} We therefore focus in this section on online responses---``likes" and ``retweets" by ordinary Twitter users of messages composed or shared by our celebrities---that allow us to differentiate responses both tweet by tweet, and also differentially depending on how a particular tweet reached a particular user. 

\subsection{Value of celebrity involvement}\label{subsec:value_endorsement}

We begin by asking whether a celebrity's influence in diffusion on social media is due simply to their reach (the size of their network) or also because when they pass on it is more likely to be subsequently passed on (the endorsement effect due to their involvement).

Our identification strategy exploits a particular feature of retweets in Twitter. A respondent $j$ who sees a retweet observes two names: the name of the original writer of the tweet, and of the person whom $j$ follows who retweeted it. Any names in between---say, a follower of the original writer who retweeted it to the person who retweeted it to $j$---are unobserved.

We exploit this feature of Twitter---that intermediaries in a retweet chain are lost---in our experimental design, as summarized in Figure \ref{fig:reach-vs-endorsement}. Consider a chain from a celebrity to some follower $F_1$ and then to some follower of this follower (who does not directly follow the celebrity) $F_2$. If the celebrity retweets the message by a Joe, and then this is retweeted by $F_1$, observe that $F_2$ sees the message, sees that it is composed by a Joe, and knows that $F_1$ retweeted it. But crucially $F_2$ does not know that the celebrity had retweeted it: $F_2$ is likely to be blind to the celebrity's involvement. On the other hand, if the celebrity had written this tweet herself rather than retweeted it, this would be visible to the $F_2$. This is depicted in Figure \ref{fig:reach-vs-endorsement}.

By randomizing whether the message is originally tweeted by the celebrity, or instead originally tweeted by a Joe and then retweeted by the celebrity, we can identify the celebrity endorsement effect by looking at $F_2$'s behavior.

To test this, we estimate, by Poisson regression, the equation 
\begin{equation}
\E[y_{tr}\vert {\bf{x}}_{tr}] = \exp\left(\alpha\cdot \text{Celeb}_{tr} + \beta \cdot \text{log(Followers)}_r + \gamma' X_t \right)
\label{eq:reach_endorse_estimating}
\end{equation}
where $t$ indexes a tweet and $r$ indexes a retweeter (i.e., an $F_1$ who retweeted the tweet $t$). Each observation is a retweet of one of our original tweets, and the dependent variable $y_{tr}$ is a count of how many times this retweet was itself either liked or retweeted again by an $F_2$. Since $y$ is a count, we estimate a Poisson regression, with robust standard errors to allow for arbitrary variance terms clustered at the original tweet ($t$) level. 
We control for the log number of followers of the $F_1$, and for various characteristics of the tweet (phase of experiment and formal vs. casual style).   
The key coefficient of interest is $\alpha$, which measures the differential impact of the tweet having been written by the celebrity and this being observable to the $F_2$-level person making the decision to retweet. 

Table \ref{tab:celeb_v_org_v_joe_F2} presents our results. As discussed in more detail in Section \ref{subsec:onlinedata} above, we have three main outcome variables: (1) whether the agent either liked or retweeted the tweet,  (2) whether an agent liked the tweet, and (3) whether an agent retweeted the tweet.  Columns 1, 3, and 5 present the results on the full sample for each of these dependent variables.

We see large endorsement effects. Having a celebrity compose and tweet the message relative to having a Joe compose the message and the celebrity retweeting it leads to a 2.7-fold % = exp(1.003)
increase in the retweet or like rate (column 1, $p < 0.01$; note that since this is a Poisson model, the coefficients are interpretatble as the change in log number of retweets) by followers-of-followers ($F_2$s) . The results are similar when we look at likes or retweets alone. 

These results imply that, holding the content of the tweet constant (since it is randomized across tweets) and holding the $F_2$ position in the network constant (since they are all followers-of-followers of the celebrity), having the $F_2$ be aware of the celebrity's involvement in passing the message almost triples the likelihood that the $F_2$ responds online.

There are, however, two main potential threats to identification here. The first is that when we look at $F_2$ agents, i.e., those who are at distance two from the celebrity of interest, whether a given agent sees a retweet from his or her $F_1$'s may be endogenous and respond to our treatment. Namely, which $F_1$s choose to retweet the message may be directly affected by the fact that the celebrity composed the message, rather than retweeting it from a Joe. In equation \ref{eq:reach_endorse_estimating}, we always control for the log number of followers of the $F_1$ who retweeted the message, and hence the number of $F_2$s who could potentially retweet it, so there is no mechanical reason there would be a bias in equation \ref{eq:reach_endorse_estimating}. But there may nevertheless be a \emph{compositional} difference in which $F_1$'s retweet it, which could potentially lead to selection bias in terms of which $F_2$s are more likely to see the retweet in the first place. 

To address this issue, in Phase III of the experiment, we added an additional randomization. Specifically, in Phase III of the experiment we use the subset of Joes who are also $F_1$s, and so direct followers of our celebrities. For some of these Joes, we randomly had their accounts retweet our celebrities' tweets and retweets in the experiment. For this sample, we can look at how \emph{their} followers---that is, the followers of $F_1$ Joe's we exogenously forced to retweet a particular tweet---responded as we randomly vary whether the celebrity, an organization, or a Joe composes the message. We analyze this experiment by estimating equation (\ref{eq:reach_endorse_estimating}) just as we did for the full sample of $F_2$s, but for this sample we have the advantage that whether an $F_2$ sees the tweet is guaranteed to be exogenous by construction.

Columns 2, 4, and 6 present the results. The point estimates are very similar to those in the full sample, and we cannot reject that any of the point estimates are different. Note that we lose a lot of power, so we cannot reject zero in this sub-sample as well ($p = 0.268$), but the fact that the point estimates are so similar to the overall effects in columns 1, 3, and 5 provides some suggestive evidence that the possible endogenous selection of $F_1$s in our whole sample is not leading to substantial bias.

The second potential confound comes from the fact that a retweet carries with it information about how many times the original tweet has been retweeted or liked as of the time the user views it (see Figure \ref{fig:example}, which shows the number of retweets next to the arrow graphic and the number of likes next to the heart graphic). One may worry then that since our treatment assignment affects the retweet count, this itself could spur further changes in the likelihood of retweeting. The same Phase III randomization of forced Joe retweets also helps us address this issue, because we randomly varied the number of Joes we forced to retween a particular tweet. In Appendix \ref{sec:rt_count}, Table \ref{tab:exjoegroup_F1_F2} presents a Poisson regressions of retweets and likes on the number of Joes that were forced to retweet a given celebrity's tweet or retweet. (This is of course net of the forced Joes' behavior.) What we find is that being randomly assigned one, five, ten, or even fifteen extra retweets makes no impact on the number of $F_1$ or $F_2$ retweets that the given tweet faces.

Taken together, our results suggest that an agent who knows that the message was composed by an authority in the sense of a celebrity as compared to thinking it is a random individual is 2.7 times 
more likely to retweet or like the tweet. This indicates that there is a large endorsement effect.

\subsection{Value of celebrity authorship}

The preceding analysis compared individuals who were effectively randomly blinded to whether a celebrity was or was not involved in the message composition and passing in order to estimate an endorsement effect. We next ask, for a given individual, even if they know that a celebrity is involved and endorsing the message by passing it on, is there an extra endorsement effect from knowing that the celebrity composed it as compared to simply being a conduit?

Table \ref{tab:celeb_v_org_v_joe_F1} presents the results of Poisson regressions at the tweet level. That is, we now restrict to direct followers of the celebrity ($F_1$ individuals), and estimate
\begin{equation}
\E[y_{t}\vert {\bf x}_{t}] = \exp\left(\alpha \cdot \text{Celeb}_{t} + \beta \cdot \text{log(Followers)}_t + \gamma' X_t \right).
\label{eq:reach_endorse_estimating_f1}
\end{equation}
We now have one observation per tweet, and look at the number of retweets/likes, retweets, or likes by $F_1$ agents who are distance 1 from the celebrity passing along the tweet. We are interested in whether the tweet being randomly assigned to be composed by the Joe versus the celebrity leads to a higher retweet rate. 

We find evidence of a large endorsement through authorship effect for celebrities with the retweet/like rate increasing 2.9-fold % = exp(1.077)
(column 1, $p<0.01$). In fact, an agent who observes a tweet composed from the celebrity rather than a retweet of a Joe is 2.2 times %= exp(0.781)
more likely to like the tweet (column 2, $p=0.00$) and 3.66 times % = exp(1.298) 
more likely to retweet the tweet (column 3, $p = 0.00$).




\subsection{Value of source citation}

The next question to ask is whether including source citation increases diffusive behavior.  Source citations come in several forms. First, sources are simply provided though there is no verifiable references. This is of the form ``Did you know that according to WHO, Hep B vaccine is the first vaccine to prevent cancer that is liver cancer?'' Second, sources are cited, and there is a Google shortened link provided.\footnote{Note that Twitter automatically produces a short preview of the content if the site linked to has Twitter cards set up. There is one non-Google shortened link used when citing IDAI (Ikatan Dokter Anak Indonesia, the Indonesian Pediatric Society).}


To examine this question, we re-estimate equation \eqref{eq:reach_endorse_estimating_f1} at the $F_1$ level, but also add a variable that captures whether the tweet was randomly selected to include a source.\footnote{Note that the number of observations is smaller here, because some tweets on topics deemed 'sensitive' by the Government always included a source, as we noted above. We restrict the analysis here to those tweets for which we randomized whether the source was included or not.} Table \ref{tab:credboost_F1} presents the results. Columns 1-4 look at pooled likes and retweets, 5-8 look at retweets, and 9-12 look at likes. We also condition the regressions to the sample where the celebrity retweets the Joe (columns 2, 6, 10), the celebrity directly tweets (columns 3, 7, 11), and the celebrity retweets an organization (columns 4, 8, 12).

On average, pooling across all messaging configurations we find that source citation reduces the retweet and liking rate by 24.7 percent  ($p = 0.12$). % 1-exp(-0.284)
This is particularly driven by reduced retweeting behavior (a decline of 26.8 percent, $p = 0.095$). %1-exp(-0.312)
Disaggregating across whether the celebrity composed and tweeted the message or retweeted a Joe or an organization, we find that the large reductions in retweet rates persist when a Joe composed the message (a 40.7 percent  decline, $p = 0.047$) %1-exp(-0.523)
or when the celebrity directly tweets the message (a 29.5 percent  decline, $p = 0.002$).  %1-exp(-0.349)
Sources only cease to have an adverse effect  and wind up having no effect when an organization itself (here health based organizations) tweets the message which is consistent with the idea that the organization itself is essentially interpreted as a source. 

In sum, for both Joes and  celebrities, including a source in tweets ultimately depresses retweet rates and the extent of diffusion.



\subsection{Value of multiple exposures}

Lastly we look at the role of multiple exposures versus a single exposure. In models of diffusion there is a contrast between ``simple'' and ``complex'' contagion models, both of which are extensively studied. The distinction matters for the design of campaigns aiming to maximize diffusion.  In simple contagion, adoption happens at the point of a single exposure to the information.  In contrast, there are ``complex contagion'' models, wherein an individual must have multiple exposures before adoption \citep*{centola2007complex,romero2011differences,ghasemiesfeh2013complex}.\footnote{A micro-foundation for complex contagion-like behavior is as follows:  consider a Bayesian individual who is unsure about whether it is worthwhile to tweet or retweet about immunization. Her default is to not tweet: she only tweets or retweets if she is sure enough that it is worthwhile, because say there is a small cost to passing on a message that is not worth it. In this case, she only acts when she is sure enough; with enough exposures she may clear the threshold and then act, and at that point a marginal exposure should not matter.}  \cite*{beaman2016can} provide evidence in favor of complex contagion in a different setting---that of technological adoption in rural networks. 
While the networks literature across myriad disciplines (e.g., computer science, applied math, sociology, economics) have different perspecives on why this may be the case, roughly speaking complex contagion processes differ from simple contagion processes in that there is a premium for identifying central individuals. This makes it considerably more likely that a given individual in the network receives multiple exposures and thereby affects the odds of something going viral.



To get at these issues, we look at whether there are linear or non-linear effects to exposure to a message.   
Table \ref{tab:panel_daylevel_exposure} presents a Poisson regression to examine the shape of the response function. We look at all agents at the $F_1$ level, who are followers of our celebrity in question, and the observation is at the user-date level. We ask how the number of retweets of our campaign's tweets that they see from celebrities they follow on that day by the agent depends on the (randomly assigned) exposure to tweets on the given day. Since celebrities are only assigned to tweet once per day, multiple signals will come from users who follow multiple celebrities. Further, because we are interested in non-linear effects, we condition on a sample who follow at least 3 celebrities. We estimate a regression of the form

\begin{equation}
\E [y_{id} \vert {\bf x}_{id}] = \exp \left( \alpha + \sum_{k=2}^K \beta_k {\bf 1}\{\text{Exposure to }k\text{ tweets today}_{id}\} + \mu_i + \mu_d \right),
\label{eq:exposure}
\end{equation}
where $y_{id}$ is the number of retweets that an $F_1$ individual $i$ makes on date $d$ out of the set of campaign tweets that he is directly exposed to from celebrities he follows and which includes user and date fixed effects. 


Going from 1 exposure to 2 exposures leads to just over a two-fold increase in the retweet rate or a 110 percent  % = exp(0.74)
increase in the retweet rate ($p = 0.01$). That there is an effect suggests that we are not in a world of simple contagion. Then going from 1 to 3 corresponds to a 2.6-fold or 160 percent  increase in the retweet rate ($p = 0.08$).  Finally going to 4-7 exposures leads to no differential retweet rate relative to 1, though the point estimate is large but noisily estimated. This clearly rejects a linear effect model: the first additional exposure contributes to the largest increase in the retweet rate, the second additional tweet has additional value,  and there is no effect for marginal exposures, which indicates concavity.



This suggests the shape function begins linearly and then flattens out. This is inconsistent with simple contagion. Moreover, notice this is also inconsistent with a model of attention where an agent randomly checks her phone and then decides to retweet, since in this case the retweet count should scale linearly, but in fact it is concave.

Ultimately, the evidence is consistent with a complex contagion-like model that having multiple tacit endorsements is enough to make it worthwhile for the user to behave. This is particularly important because the theory demonstrates that there is a striking difference in whether a policymaker must strive to contact the ``right'' individuals (central individuals) or not---complex contagion models have a premium in seeding information with influential. The data then shows that even without the endorsement effect itself, seeding influential individuals with information would have more value simply through the fact that it would generate more multiple exposures.



\subsection{Discussion}


In this section we have studied how endorsement effects of various kinds may influence consumption of and passing on information. The results are nuanced. Our design allows us to parse the endorsement effect of a celebrity from the reach effect, and using this approach, we find the endorsement effect per se to be large: both likes and retweets increase considerably when a celebrity is randomly assigned to write the same message as a Joe. At the same time, inclusion of credible sourcing in the message does not help: on average it reduces retweeting. Further exposures themselves do matter, contrary to common views on diffusion, but in a concave way. Multiple exposures help at the outset but subsequently decline in marginal value.

This suggests certain important themes to focus on in future studies of diffusion. First, more attention ought to be paid to  ``node identity''---that is, who is involved in writing or passing the information and at what stage. This plays an enormous role in our setting, as having the celebrity be the source plays an outsized role per se. This type of concern is often swept aside, due to the obvious complexities, in typical studies of diffusion. A notable exception is \cite{beaman2018diffusion}, who focus on how the gender of the individual in the network strongly affects diffusion of information. Second, the results suggest certain types of diffusion are more likely: in this case multiple exposures (closer in spirit to complex contagion) plays a crucial role, in keeping with recent work in other contexts (e.g., \cite{beaman2016can} for technology adoption). Third, the extent of diffusion itself, typically parametrized either by time or the intrinsic virality of the information, may greatly depend on the topic. While taken for granted, there is limited research in terms of how we expect diffusion to differ by content-type and how this interacts with both the \emph{who} and the \emph{how much}. 



==> ecta.bst.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Econometrica bibliography style,  
%%%
%%% for use with LaTeX2e and Natbib (or chicago), named style following the 
%%% recommendations of Fudenberg and Hodges (1997), 
%%% Econometrica Vol. 65, N. 4, pp. 965--975,
%%% found at http://www.econometricsociety.org/manual/manual.html
%%% for submission to Econometrica.
%%% 
%%% by Sebastian Perez-Duarte, perez@ensae.fr (2000)
%%% 
%%% Based on Makebst by Patrick Daly
%%%  
%%%%%%%%%%%%%%%%%%%%%%%%%%% SUMMARY %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%% Compared to the bst file econometrica.bst (by KC Border), the present
%%% style file is closer to the canonical way of presenting the list of 
%%% references in Econometrica, a publication of the Econometric Society.
%%% 
%%% The main differences are: the format of the address, the absence of number 
%%% in articles.
%%%%%%%%%%%%%%%%%%%%%%%%%%%% LICENSE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% This generated file can be redistributed and/or modified under the terms
%%% of the LaTeX Project Public License Distributed from CTAN
%%% archives in directory macros/latex/base/lppl.txt; either
%%% version 1 of the License, or any later version.
%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%% END %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% This is file `ecta.bst',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% merlin.mbs  (with options: `ay,cay,nm-rev1,nmdash,nmft,nmft-sc,keyxyr,dt-beg,yr-par,yrp-col,note-yr,tit-qq,atit-u,thtit-a,vnum-x,volp-com,num-xser,bkpg-x,add-pub,pre-pub,edby,blk-com,ppx,ed,abr,ednx,xedn,nfss')
%% ----------------------------------------
%% *** Econometrica -- close ***
%% 
%% Copyright 1994-2000 Patrick W Daly
 % ===============================================================
 % IMPORTANT NOTICE:
 % This bibliographic style (bst) file has been generated from one or
 % more master bibliographic style (mbs) files, listed above.
 %
 % This generated file can be redistributed and/or modified under the terms
 % of the LaTeX Project Public License Distributed from CTAN
 % archives in directory macros/latex/base/lppl.txt; either
 % version 1 of the License, or any later version.
 % ===============================================================
 % Name and version information of the main mbs file:
 % \ProvidesFile{merlin.mbs}[2000/05/04 4.01 (PWD, AO, DPC)]
 %   For use with BibTeX version 0.99a or later
 %-------------------------------------------------------------------
 % This bibliography style file is intended for texts in ENGLISH
 % This is an author-year citation style bibliography. As such, it is
 % non-standard LaTeX, and requires a special package file to function properly.
 % Such a package is    natbib.sty   by Patrick W. Daly
 % or:                  chicago.sty
 % The form of the bibitem entries is
 %   \bibitem[\protect\citeauthoryear{Jones, Baker, and Smith}
 %        {Jones et al.}{1990}{key}...
 %---------------------------------------------------------------------

ENTRY
  { address
    author
    booktitle
    chapter
    edition
    editor
    howpublished
    institution
    journal
    key
    month
    note
    number
    organization
    pages
    publisher
    school
    series
    title
    type
    volume
    year
  }
  {}
  { label extra.label sort.label short.list }
INTEGERS { output.state before.all mid.sentence after.sentence after.block }
FUNCTION {init.state.consts}
{ #0 'before.all :=
  #1 'mid.sentence :=
  #2 'after.sentence :=
  #3 'after.block :=
}
STRINGS { s t}
FUNCTION {output.nonnull}
{ 's :=
  output.state mid.sentence =
    { ", " * write$ }
    { output.state after.block =
        { add.period$ write$
          newline$
          "\newblock " write$
        }
        { output.state before.all =
            'write$
            { add.period$ " " * write$ }
          if$
        }
      if$
      mid.sentence 'output.state :=
    }
  if$
  s
}
FUNCTION {output}
{ duplicate$ empty$
    'pop$
    'output.nonnull
  if$
}
FUNCTION {output.check}
{ 't :=
  duplicate$ empty$
    { pop$ "empty " t * " in " * cite$ * warning$ }
    'output.nonnull
  if$
}
FUNCTION {fin.entry}
{ add.period$
  write$
  newline$
}

FUNCTION {new.block}
{ output.state before.all =
    'skip$
    { after.block 'output.state := }
  if$
}
FUNCTION {new.sentence}
{ output.state after.block =
    'skip$
    { output.state before.all =
        'skip$
        { after.sentence 'output.state := }
      if$
    }
  if$
}
FUNCTION {add.blank}
{  " " * before.all 'output.state :=
}

FUNCTION {date.block}
{
  ":" *
  add.blank
}

FUNCTION {not}
{   { #0 }
    { #1 }
  if$
}
FUNCTION {and}
{   'skip$
    { pop$ #0 }
  if$
}
FUNCTION {or}
{   { pop$ #1 }
    'skip$
  if$
}
FUNCTION {non.stop}
{ duplicate$
   "}" * add.period$
   #-1 #1 substring$ "." =
}

FUNCTION {new.block.checkb}
{ empty$
  swap$ empty$
  and
    'skip$
    'new.block
  if$
}
FUNCTION {field.or.null}
{ duplicate$ empty$
    { pop$ "" }
    'skip$
  if$
}
FUNCTION {emphasize}
{ duplicate$ empty$
    { pop$ "" }
    { "\emph{" swap$ * "}" * }
  if$
}
FUNCTION {scaps}
{ duplicate$ empty$
    { pop$ "" }
    { "\textsc{" swap$ * "}" * }
  if$
}
FUNCTION {bib.name.font}
{ scaps }
FUNCTION {bib.fname.font}
{ bib.name.font }
FUNCTION {tie.or.space.prefix}
{ duplicate$ text.length$ #3 <
    { "~" }
    { " " }
  if$
  swap$
}

FUNCTION {capitalize}
{ "u" change.case$ "t" change.case$ }

FUNCTION {space.word}
{ " " swap$ * " " * }
 % Here are the language-specific definitions for explicit words.
 % Each function has a name bbl.xxx where xxx is the English word.
 % The language selected here is ENGLISH
FUNCTION {bbl.and}
{ "and"}

FUNCTION {bbl.etal}
{ "et~al." }

FUNCTION {bbl.editors}
{ "eds." }

FUNCTION {bbl.editor}
{ "ed." }

FUNCTION {bbl.edby}
{ "ed. by" }

FUNCTION {bbl.edition}
{ "ed." }

FUNCTION {bbl.volume}
{ "vol." }

FUNCTION {bbl.of}
{ "of" }

FUNCTION {bbl.number}
{ "no." }

FUNCTION {bbl.nr}
{ "no." }

FUNCTION {bbl.in}
{ "in" }

FUNCTION {bbl.pages}
{ "" }

FUNCTION {bbl.page}
{ "" }

FUNCTION {bbl.chapter}
{ "chap." }

FUNCTION {bbl.techrep}
{ "Tech. Rep." }

FUNCTION {bbl.mthesis}
{ "Master's thesis" }

FUNCTION {bbl.phdthesis}
{ "Ph.D. thesis" }

MACRO {jan} {"Jan."}

MACRO {feb} {"Feb."}

MACRO {mar} {"Mar."}

MACRO {apr} {"Apr."}

MACRO {may} {"May"}

MACRO {jun} {"Jun."}

MACRO {jul} {"Jul."}

MACRO {aug} {"Aug."}

MACRO {sep} {"Sep."}

MACRO {oct} {"Oct."}

MACRO {nov} {"Nov."}

MACRO {dec} {"Dec."}

MACRO {acmcs} {"ACM Computing Surveys"}

MACRO {acta} {"Acta Informatica"}

MACRO {cacm} {"Communications of the ACM"}

MACRO {ibmjrd} {"IBM Journal of Research and Development"}

MACRO {ibmsj} {"IBM Systems Journal"}

MACRO {ieeese} {"IEEE Transactions on Software Engineering"}

MACRO {ieeetc} {"IEEE Transactions on Computers"}

MACRO {ieeetcad}
 {"IEEE Transactions on Computer-Aided Design of Integrated Circuits"}

MACRO {ipl} {"Information Processing Letters"}

MACRO {jacm} {"Journal of the ACM"}

MACRO {jcss} {"Journal of Computer and System Sciences"}

MACRO {scp} {"Science of Computer Programming"}

MACRO {sicomp} {"SIAM Journal on Computing"}

MACRO {tocs} {"ACM Transactions on Computer Systems"}

MACRO {tods} {"ACM Transactions on Database Systems"}

MACRO {tog} {"ACM Transactions on Graphics"}

MACRO {toms} {"ACM Transactions on Mathematical Software"}

MACRO {toois} {"ACM Transactions on Office Information Systems"}

MACRO {toplas} {"ACM Transactions on Programming Languages and Systems"}

MACRO {tcs} {"Theoretical Computer Science"}
FUNCTION {bibinfo.check}
{ swap$
  duplicate$ missing$
    {
      pop$ pop$
      ""
    }
    { duplicate$ empty$
        {
          swap$ pop$
        }
        { swap$
          pop$
        }
      if$
    }
  if$
}
FUNCTION {bibinfo.warn}
{ swap$
  duplicate$ missing$
    {
      swap$ "missing " swap$ * " in " * cite$ * warning$ pop$
      ""
    }
    { duplicate$ empty$
        {
          swap$ "empty " swap$ * " in " * cite$ * warning$
        }
        { swap$
          pop$
        }
      if$
    }
  if$
}
STRINGS  { bibinfo}
INTEGERS { nameptr namesleft numnames }

FUNCTION {format.names}
{ 'bibinfo :=
  duplicate$ empty$ 'skip$ {
  's :=
  "" 't :=
  #1 'nameptr :=
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { s nameptr
      duplicate$ #1 >
        { "{f.~}{vv~}{ll}{, jj}" }
        { "{vv~}{ll}{, jj}{, f.}" }
      if$
      format.name$
      bibinfo bibinfo.check
      't :=
      nameptr #1 >
        {
          namesleft #1 >
            { ", " * t * }
            {
              numnames #2 >
                { "," * }
                'skip$
              if$
              s nameptr "{ll}" format.name$ duplicate$ "others" =
                { 't := }
                { pop$ }
              if$
              t "others" =
                {
                  " " * bbl.etal *
                  bib.name.font
                }
                {
                  bbl.and
                  space.word * t *
                }
              if$
            }
          if$
        }
        't
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
  t "others" =
    'skip$
    { bib.name.font }
  if$
  } if$
}
FUNCTION {format.names.ed}
{
  'bibinfo :=
  duplicate$ empty$ 'skip$ {
  's :=
  "" 't :=
  #1 'nameptr :=
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { s nameptr
      "{f.~}{vv~}{ll}{, jj}"
      format.name$
      bibinfo bibinfo.check
      't :=
      nameptr #1 >
        {
          namesleft #1 >
            { ", " * t * }
            {
              numnames #2 >
                { "," * }
                'skip$
              if$
              s nameptr "{ll}" format.name$ duplicate$ "others" =
                { 't := }
                { pop$ }
              if$
              t "others" =
                {

                  " " * bbl.etal *
                }
                {
                  bbl.and
                  space.word * t *
                }
              if$
            }
          if$
        }
        't
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
  } if$
}
FUNCTION {format.key}
{ empty$
    { key field.or.null }
    { "" }
  if$
}

FUNCTION {format.authors}
{ author "author" format.names
}
FUNCTION {get.bbl.editor}
{ editor num.names$ #1 > 'bbl.editors 'bbl.editor if$ }

FUNCTION {format.editors}
{ editor "editor" format.names duplicate$ empty$ 'skip$
    {
      "," *
      " " *
      get.bbl.editor
      *
    }
  if$
}
FUNCTION {format.note}
{
 note empty$
    { "" }
    { note #1 #1 substring$
      duplicate$ "{" =
        'skip$
        { output.state mid.sentence =
          { "l" }
          { "u" }
        if$
        change.case$
        }
      if$
      note #2 global.max$ substring$ * "note" bibinfo.check
    }
  if$
}

FUNCTION {format.title}
{ title
  "title" bibinfo.check
  duplicate$ empty$ 'skip$
    {
      "\enquote{" swap$ *
      non.stop
        { ",} " * }
        { "} " * }
      if$
    }
  if$
}
FUNCTION {end.quote.title}
{ title empty$
    'skip$
    { before.all 'output.state := }
  if$
}
FUNCTION {format.full.names}
{'s :=
 "" 't :=
  #1 'nameptr :=
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { s nameptr
      "{vv~}{ll}" format.name$
      't :=
      nameptr #1 >
        {
          namesleft #1 >
            { ", " * t * }
            {
              s nameptr "{ll}" format.name$ duplicate$ "others" =
                { 't := }
                { pop$ }
              if$
              t "others" =
                {
                  " " * bbl.etal *
                }
                {
                  numnames #2 >
                    { "," * }
                    'skip$
                  if$
                  bbl.and
                  space.word * t *
                }
              if$
            }
          if$
        }
        't
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
}

FUNCTION {author.editor.key.full}
{ author empty$
    { editor empty$
        { key empty$
            { cite$ #1 #3 substring$ }
            'key
          if$
        }
        { editor format.full.names }
      if$
    }
    { author format.full.names }
  if$
}

FUNCTION {author.key.full}
{ author empty$
    { key empty$
         { cite$ #1 #3 substring$ }
          'key
      if$
    }
    { author format.full.names }
  if$
}

FUNCTION {editor.key.full}
{ editor empty$
    { key empty$
         { cite$ #1 #3 substring$ }
          'key
      if$
    }
    { editor format.full.names }
  if$
}

FUNCTION {make.full.names}
{ type$ "book" =
  type$ "inbook" =
  or
    'author.editor.key.full
    { type$ "proceedings" =
        'editor.key.full
        'author.key.full
      if$
    }
  if$
}

FUNCTION {output.bibitem}
{ newline$
  "\bibitem[" write$
  "\protect\citeauthoryear{" make.full.names * "}{" * write$
  label write$
  "}{" year duplicate$ empty$
    { pop$ "????" }
    'skip$
  if$
  * extra.label * "}]{" * write$
  cite$ write$
  "}" write$
  newline$
  ""
  before.all 'output.state :=
}

FUNCTION {n.dashify}
{
  't :=
  ""
    { t empty$ not }
    { t #1 #1 substring$ "-" =
        { t #1 #2 substring$ "--" = not
            { "--" *
              t #2 global.max$ substring$ 't :=
            }
            {   { t #1 #1 substring$ "-" = }
                { "-" *
                  t #2 global.max$ substring$ 't :=
                }
              while$
            }
          if$
        }
        { t #1 #1 substring$ *
          t #2 global.max$ substring$ 't :=
        }
      if$
    }
  while$
}

FUNCTION {word.in}
{ bbl.in
  " " * }

FUNCTION {format.date}
{ year "year" bibinfo.check duplicate$ empty$
    {
      "empty year in " cite$ * "; set to ????" * warning$
       pop$ "????"
    }
    'skip$
  if$
  extra.label *
  before.all 'output.state :=
  " (" swap$ * ")" *
}
FUNCTION {format.btitle}
{ title "title" bibinfo.check
  duplicate$ empty$ 'skip$
    {
      emphasize
    }
  if$
}
FUNCTION {either.or.check}
{ empty$
    'pop$
    { "can't use both " swap$ * " fields in " * cite$ * warning$ }
  if$
}
FUNCTION {format.bvolume}
{ volume empty$
    { "" }
    { bbl.volume volume tie.or.space.prefix
      "volume" bibinfo.check * *
      series "series" bibinfo.check
      duplicate$ empty$ 'pop$
        { swap$ bbl.of space.word * swap$
          emphasize * }
      if$
      "volume and number" number either.or.check
    }
  if$
}
FUNCTION {format.number.series}
{ volume empty$
    { number empty$
        { series field.or.null }
        { series empty$
            { number "number" bibinfo.check }
        { output.state mid.sentence =
            { bbl.number }
            { bbl.number capitalize }
          if$
          number tie.or.space.prefix "number" bibinfo.check * *
          bbl.in space.word *
          series "series" bibinfo.check *
        }
      if$
    }
      if$
    }
    { "" }
  if$
}

FUNCTION {format.edition}
{ edition duplicate$ empty$ 'skip$
    {
      output.state mid.sentence =
        { "l" }
        { "t" }
      if$ change.case$
      "edition" bibinfo.check
      " " * bbl.edition *
    }
  if$
}
INTEGERS { multiresult }
FUNCTION {multi.page.check}
{ 't :=
  #0 'multiresult :=
    { multiresult not
      t empty$ not
      and
    }
    { t #1 #1 substring$
      duplicate$ "-" =
      swap$ duplicate$ "," =
      swap$ "+" =
      or or
        { #1 'multiresult := }
        { t #2 global.max$ substring$ 't := }
      if$
    }
  while$
  multiresult
}
FUNCTION {format.pages}
{ pages duplicate$ empty$ 'skip$
    { duplicate$ multi.page.check
        {
          n.dashify
        }
        {
        }
      if$
      "pages" bibinfo.check
    }
  if$
}
FUNCTION {format.journal.pages}
{ pages duplicate$ empty$ 'pop$
    { swap$ duplicate$ empty$
        { pop$ pop$ format.pages }
        {
          ", " *
          swap$
          n.dashify
          "pages" bibinfo.check
          *
        }
      if$
    }
  if$
}
FUNCTION {format.vol.num.pages}
{ volume field.or.null
  duplicate$ empty$ 'skip$
    {
      "volume" bibinfo.check
    }
  if$
  format.journal.pages
}

FUNCTION {format.chapter.pages}
{ chapter empty$
    'format.pages
    { type empty$
        { bbl.chapter }
        { type "l" change.case$
          "type" bibinfo.check
        }
      if$
      chapter tie.or.space.prefix
      "chapter" bibinfo.check
      * *
      pages empty$
        'skip$
        { ", " * format.pages * }
      if$
    }
  if$
}

FUNCTION {format.booktitle}
{
  booktitle "booktitle" bibinfo.check
  emphasize
}
FUNCTION {format.in.ed.booktitle}
{ format.booktitle duplicate$ empty$ 'skip$
    {
      editor "editor" format.names.ed duplicate$ empty$ 'pop$
        {
          bbl.edby
          " " * swap$ *
          swap$
          "," *
          " " * swap$
          * }
      if$
      word.in swap$ *
    }
  if$
}
FUNCTION {format.thesis.type}
{ type duplicate$ empty$
    'pop$
    { swap$ pop$
      "t" change.case$ "type" bibinfo.check
    }
  if$
}
FUNCTION {format.tr.number}
{ number "number" bibinfo.check
  type duplicate$ empty$
    { pop$ bbl.techrep }
    'skip$
  if$
  "type" bibinfo.check
  swap$ duplicate$ empty$
    { pop$ "t" change.case$ }
    { tie.or.space.prefix * * }
  if$
}
FUNCTION {format.article.crossref}
{
  word.in
  " \cite{" * crossref * "}" *
}
FUNCTION {format.book.crossref}
{ volume duplicate$ empty$
    { "empty volume in " cite$ * "'s crossref of " * crossref * warning$
      pop$ word.in
    }
    { bbl.volume
      swap$ tie.or.space.prefix "volume" bibinfo.check * * bbl.of space.word *
    }
  if$
  " \cite{" * crossref * "}" *
}
FUNCTION {format.incoll.inproc.crossref}
{
  word.in
  " \cite{" * crossref * "}" *
}
FUNCTION {format.org.or.pub}
{ 't :=
  ""
  address empty$ t empty$ and
    'skip$
    {
      address "address" bibinfo.check *
      t empty$
        'skip$
        { address empty$
            'skip$
            { ": " * }
          if$
          t *
        }
      if$
    }
  if$
}
FUNCTION {format.publisher.address}
{ publisher "publisher" bibinfo.warn format.org.or.pub
}

FUNCTION {format.organization.address}
{ organization "organization" bibinfo.check format.org.or.pub
}

STRINGS {oldname}

FUNCTION {name.or.dash}
{ 's :=
   oldname empty$
     { s 'oldname := s }
     { s oldname =
%         { "---" }   old style
         { "---\hspace{-.1pt}---\hspace{-.1pt}---" }    
%SPD 2000
         { s 'oldname := s }
       if$
     }
   if$
}

FUNCTION {article}
{ output.bibitem
  format.authors "author" output.check
  author format.key output
  name.or.dash
  format.date "year" output.check
  date.block
  format.title "title" output.check
  end.quote.title
  crossref missing$
    {
      journal
      "journal" bibinfo.check
      emphasize
      "journal" output.check
      format.vol.num.pages output
    }
    { format.article.crossref output.nonnull
      format.pages output
    }
  if$
  format.note output
  fin.entry
}
FUNCTION {book}
{ output.bibitem
  author empty$
    { format.editors "author and editor" output.check
      editor format.key output
      name.or.dash
    }
    { format.authors output.nonnull
      name.or.dash
      crossref missing$
        { "author and editor" editor either.or.check }
        'skip$
      if$
    }
  if$
  format.date "year" output.check
  date.block
  format.btitle "title" output.check
  crossref missing$
    { format.bvolume output
      format.number.series output
      format.publisher.address output
    }
    {
      format.book.crossref output.nonnull
    }
  if$
  format.edition output
  format.note output
  fin.entry
}
FUNCTION {booklet}
{ output.bibitem
  format.authors output
  author format.key output
  name.or.dash
  format.date "year" output.check
  date.block
  format.title "title" output.check
  end.quote.title
  howpublished "howpublished" bibinfo.check output
  address "address" bibinfo.check output
  format.note output
  fin.entry
}

FUNCTION {inbook}
{ output.bibitem
  author empty$
    { format.editors "author and editor" output.check
      editor format.key output
      name.or.dash
    }
    { format.authors output.nonnull
      name.or.dash
      crossref missing$
        { "author and editor" editor either.or.check }
        'skip$
      if$
    }
  if$
  format.date "year" output.check
  date.block
  format.btitle "title" output.check
  crossref missing$
    {
      format.publisher.address output
      format.bvolume output
      format.chapter.pages "chapter and pages" output.check
      format.number.series output
    }
    {
      format.chapter.pages "chapter and pages" output.check
      format.book.crossref output.nonnull
    }
  if$
  format.edition output
  format.note output
  fin.entry
}

FUNCTION {incollection}
{ output.bibitem
  format.authors "author" output.check
  author format.key output
  name.or.dash
  format.date "year" output.check
  date.block
  format.title "title" output.check
  end.quote.title
  crossref missing$
    { format.in.ed.booktitle "booktitle" output.check
      format.publisher.address output
      format.bvolume output
      format.number.series output
      format.chapter.pages output
      format.edition output
    }
    { format.incoll.inproc.crossref output.nonnull
      format.chapter.pages output
    }
  if$
  format.note output
  fin.entry
}
FUNCTION {inproceedings}
{ output.bibitem
  format.authors "author" output.check
  author format.key output
  name.or.dash
  format.date "year" output.check
  date.block
  format.title "title" output.check
  end.quote.title
  crossref missing$
    { format.in.ed.booktitle "booktitle" output.check
      publisher empty$
        { format.organization.address output }
        { organization "organization" bibinfo.check output
          format.publisher.address output
        }
      if$
      format.bvolume output
      format.number.series output
      format.pages output
    }
    { format.incoll.inproc.crossref output.nonnull
      format.pages output
    }
  if$
  format.note output
  fin.entry
}
FUNCTION {conference} { inproceedings }
FUNCTION {manual}
{ output.bibitem
  format.authors output
  author format.key output
  name.or.dash
  format.date "year" output.check
  date.block
  format.btitle "title" output.check
  organization "organization" bibinfo.check output
  address "address" bibinfo.check output
  format.edition output
  format.note output
  fin.entry
}

FUNCTION {mastersthesis}
{ output.bibitem
  format.authors "author" output.check
  author format.key output
  name.or.dash
  format.date "year" output.check
  date.block
  format.title
  "title" output.check
  end.quote.title
  bbl.mthesis format.thesis.type output.nonnull
  school "school" bibinfo.warn output
  address "address" bibinfo.check output
  format.note output
  fin.entry
}

FUNCTION {misc}
{ output.bibitem
  format.authors output
  author format.key output
  name.or.dash
  format.date "year" output.check
  date.block
  format.title output
  end.quote.title
  howpublished "howpublished" bibinfo.check output
  format.note output
  fin.entry
}
FUNCTION {phdthesis}
{ output.bibitem
  format.authors "author" output.check
  author format.key output
  name.or.dash
  format.date "year" output.check
  date.block
  format.title
  "title" output.check
  end.quote.title
  bbl.phdthesis format.thesis.type output.nonnull
  school "school" bibinfo.warn output
  address "address" bibinfo.check output
  format.note output
  fin.entry
}

FUNCTION {proceedings}
{ output.bibitem
  format.editors output
  editor format.key output
  name.or.dash
  format.date "year" output.check
  date.block
  format.btitle "title" output.check
  format.bvolume output
  format.number.series output
  publisher empty$
    { format.organization.address output }
    { organization "organization" bibinfo.check output
      format.publisher.address output
    }
  if$
  format.note output
  fin.entry
}

FUNCTION {techreport}
{ output.bibitem
  format.authors "author" output.check
  author format.key output
  name.or.dash
  format.date "year" output.check
  date.block
  format.title
  "title" output.check
  end.quote.title
  format.tr.number output.nonnull
  institution "institution" bibinfo.warn output
  address "address" bibinfo.check output
  format.note output
  fin.entry
}

FUNCTION {unpublished}
{ output.bibitem
  format.authors "author" output.check
  author format.key output
  name.or.dash
  format.date "year" output.check
  date.block
  format.title "title" output.check
  end.quote.title
  format.note "note" output.check
  fin.entry
}

FUNCTION {default.type} { misc }
READ
FUNCTION {sortify}
{ purify$
  "l" change.case$
}
INTEGERS { len }
FUNCTION {chop.word}
{ 's :=
  'len :=
  s #1 len substring$ =
    { s len #1 + global.max$ substring$ }
    's
  if$
}
FUNCTION {format.lab.names}
{ 's :=
  "" 't :=
  s #1 "{vv~}{ll}" format.name$
  s num.names$ duplicate$
  #2 >
    { pop$
      " " * bbl.etal *
    }
    { #2 <
        'skip$
        { s #2 "{ff }{vv }{ll}{ jj}" format.name$ "others" =
            {
              " " * bbl.etal *
            }
            { bbl.and space.word * s #2 "{vv~}{ll}" format.name$
              * }
          if$
        }
      if$
    }
  if$
}

FUNCTION {author.key.label}
{ author empty$
    { key empty$
        { cite$ #1 #3 substring$ }
        'key
      if$
    }
    { author format.lab.names }
  if$
}

FUNCTION {author.editor.key.label}
{ author empty$
    { editor empty$
        { key empty$
            { cite$ #1 #3 substring$ }
            'key
          if$
        }
        { editor format.lab.names }
      if$
    }
    { author format.lab.names }
  if$
}

FUNCTION {editor.key.label}
{ editor empty$
    { key empty$
        { cite$ #1 #3 substring$ }
        'key
      if$
    }
    { editor format.lab.names }
  if$
}

FUNCTION {calc.short.authors}
{ type$ "book" =
  type$ "inbook" =
  or
    'author.editor.key.label
    { type$ "proceedings" =
        'editor.key.label
        'author.key.label
      if$
    }
  if$
  'short.list :=
}

FUNCTION {calc.label}
{ calc.short.authors
  short.list
  ", "
  *
  year duplicate$ empty$
  short.list key field.or.null = or
     { pop$ "" }
     'skip$
  if$
  *
  'label :=
}

FUNCTION {calc.short.label}
{ calc.short.authors short.list
  'label :=
}
FUNCTION {sort.format.names}
{ 's :=
  #1 'nameptr :=
  ""
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { s nameptr
      "{vv{ } }{ll{ }}{  f{ }}{  jj{ }}"
      format.name$ 't :=
      nameptr #1 >
        {
          "   "  *
          namesleft #1 = t "others" = and
            { "zzzzz" * }
            { t sortify * }
          if$
        }
        { t sortify * }
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
}

FUNCTION {sort.format.title}
{ 't :=
  "A " #2
    "An " #3
      "The " #4 t chop.word
    chop.word
  chop.word
  sortify
  #1 global.max$ substring$
}
FUNCTION {author.sort}
{ author empty$
    { key empty$
        { "to sort, need author or key in " cite$ * warning$
          ""
        }
        { key sortify }
      if$
    }
    { author sort.format.names }
  if$
}
FUNCTION {author.editor.sort}
{ author empty$
    { editor empty$
        { key empty$
            { "to sort, need author, editor, or key in " cite$ * warning$
              ""
            }
            { key sortify }
          if$
        }
        { editor sort.format.names }
      if$
    }
    { author sort.format.names }
  if$
}
FUNCTION {editor.sort}
{ editor empty$
    { key empty$
        { "to sort, need editor or key in " cite$ * warning$
          ""
        }
        { key sortify }
      if$
    }
    { editor sort.format.names }
  if$
}
FUNCTION {presort}
{ calc.label
  label sortify
  "    "
  *
  type$ "book" =
  type$ "inbook" =
  or
    'author.editor.sort
    { type$ "proceedings" =
        'editor.sort
        'author.sort
      if$
    }
  if$
  #1 entry.max$ substring$
  'sort.label :=
  sort.label
  *
  "    "
  *
  title field.or.null
  sort.format.title
  *
  #1 entry.max$ substring$
  'sort.key$ :=
}

ITERATE {presort}
SORT
STRINGS { last.label next.extra }
INTEGERS { last.extra.num number.label }
FUNCTION {initialize.extra.label.stuff}
{ #0 int.to.chr$ 'last.label :=
  "" 'next.extra :=
  #0 'last.extra.num :=
  #0 'number.label :=
}
FUNCTION {forward.pass}
{ last.label label =
    { last.extra.num #1 + 'last.extra.num :=
      last.extra.num int.to.chr$ 'extra.label :=
    }
    { "a" chr.to.int$ 'last.extra.num :=
      "" 'extra.label :=
      label 'last.label :=
    }
  if$
  number.label #1 + 'number.label :=
}
FUNCTION {reverse.pass}
{ next.extra "b" =
    { "a" 'extra.label := }
    'skip$
  if$
  extra.label 'next.extra :=
  extra.label
  duplicate$ empty$
    'skip$
    { "{\natexlab{" swap$ * "}}" * }
  if$
  'extra.label :=
}
EXECUTE {initialize.extra.label.stuff}
ITERATE {forward.pass}
REVERSE {reverse.pass}
FUNCTION {bib.sort.order}
{ sort.label
  "    "
  *
  year field.or.null sortify
  *
  "    "
  *
  title field.or.null
  sort.format.title
  *
  #1 entry.max$ substring$
  'sort.key$ :=
  calc.short.label
}
ITERATE {bib.sort.order}
SORT
FUNCTION {begin.bib}
{ preamble$ empty$
    'skip$
    { preamble$ write$ newline$ }
  if$
  "\begin{thebibliography}{" number.label int.to.str$ * "}" *
  write$ newline$
  "\newcommand{\enquote}[1]{``#1''}"
  write$ newline$
  "\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi"
  write$ newline$
}
EXECUTE {begin.bib}
EXECUTE {init.state.consts}
ITERATE {call.type$}
FUNCTION {end.bib}
{ newline$
  "\end{thebibliography}" write$ newline$
}
EXECUTE {end.bib}
%% End of customized bst file
%%
%% End of file `econm.bst'.

==> tab_celeb_v_org_v_joe_F1_p2.tex <==
\begin{tabular}{lccc} \hline
 & (1) & (2) & (3) \\
 & Poisson & Poisson & Poisson \\
VARIABLES & \# Pooled & \# Retweets & \# Likes \\ \hline
 &  &  &  \\
Celeb writes and tweets & 1.077 & 1.298 & 0.781 \\
 & (0.166) & (0.165) & (0.184) \\
 & [8.32e-11] & [0] & [2.19e-05] \\
 &  &  &  \\
Observations & 451 & 451 & 451 \\
Phase control & \checkmark & \checkmark & \checkmark \\
Log \#followers control & \checkmark & \checkmark & \checkmark \\
Message style control & \checkmark & \checkmark & \checkmark \\
Depvar Mean & 2.058 & 2.415 & 1.594 \\
 Joe writes and Celeb retweets log mean & 0.722 & 0.0437 & 0.0133 \\ \hline
\end{tabular}


==> tab_celeb_v_org_v_joe_F2_p2.tex <==
\begin{tabular}{lcccccc} \hline
 & (1) & (2) & (3) & (4) & (5) & (6) \\
 & Poisson & Poisson & Poisson & Poisson & Poisson & Poisson \\
VARIABLES & \# Pooled & \# Pooled & \# Retweets & \# Retweets & \# Likes & \# Likes \\ \hline
 &  &  &  &  &  &  \\
Celeb writes and tweets & 1.003 & 0.776 & 0.970 & 0.602 & 1.133 & 1.152 \\
 & (0.251) & (0.701) & (0.259) & (0.922) & (0.572) & (1.027) \\
 & [6.32e-05] & [0.268] & [0.000184] & [0.514] & [0.0476] & [0.262] \\
 &  &  &  &  &  &  \\
Observations & 1,997 & 911 & 1,997 & 911 & 1,997 & 911 \\
Phase control & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
Log \#followers control & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
Message style control & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
 Forced Joes only &  & \checkmark &  & \checkmark &  & \checkmark \\ \hline
\end{tabular}


==> tab_opinion_immun_itt_RI_lasso.tex <==
\begin{tabular}{lcccc} \hline
 & (1) & (2) & (3)   \\
 &  Ologit & Ologit & Ologit \\
VARIABLES &  Immun. Beneficial  & Immun. Safe & Immun. Important \\ \hline
 &    &  &  \\
Std. Exposure to tweets  & -0.0795 & 0.0758 & 0.0430 \\
 &   (0.0703) & (0.0637) & (0.0753) \\
 &   [0.259] & [0.234] & [0.568] \\
 &   \{.469\} & \{.611\} & \{.642\} \\
 &   &  &  \\
Observations &  2,441 & 2,441 & 2,441 \\
Potential exposure control &   \checkmark & \checkmark & \checkmark \\
Double Post-LASSO &  \checkmark & \checkmark & \checkmark \\
 Depvar Mean &  3.679 & 3.409 & 3.752 \\ \hline
\end{tabular}


==> tab_social_itt_RI_lasso.tex <==
\begin{tabular}{lcccccccc} \hline
 & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) \\
 & OLS & Poisson & Poisson & Poisson & Poisson & Poisson & Poisson & Poisson \\
VARIABLES & Total (Std) & Action Total & Forward  & Tell & RT & Other & Num. Friend & Any Friend \\ \hline
 &  &  &  &  &  &  &  &  \\
Std. Exposure to tweets & 0.0337 & 0.186 & 0.517 & 0.400 & -0.201 & 0.526 & 0.0175 & 0.000701 \\
 & (0.0339) & (0.123) & (0.256) & (0.208) & (0.237) & (0.238) & (0.0423) & (0.0581) \\
 & [0.322] & [0.132] & [0.0437] & [0.0545] & [0.396] & [0.0270] & [0.679] & [0.990] \\
 & \{.387\} & \{.206\} & \{.302\} & \{.129\} & \{.66\} & \{.124\} & \{.564\} & \{.918\} \\
 &  &  &  &  &  &  &  &  \\
Observations & 2,427 & 2,427 & 2,427 & 1,920 & 1,458 & 1,717 & 2,441 & 2,440 \\
Potential exposure control & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
Double Post-LASSO & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
 Depvar Mean & 0.00795 & 0.00795 & 0.00795 & 0.0303 & 0.0417 & 0.0406 & 0.00795 & 0.00823 \\ \hline
\end{tabular}

